Seeing with Partial Certainty: Conformal Prediction for Robotic Scene Recognition in Built Environments

In assistive robotics serving people with disabilities (PWD), accurate place recognition in built environments is crucial to ensure that robots navigate and interact safely within diverse indoor spaces. Language interfaces, particularly those powered by Large Language Models (LLM) and Vision Language Models (VLM), hold significant promise in this context, as they can interpret visual scenes and correlate them with semantic information. However, such interfaces are also known for their hallucinated predictions. In addition, language instructions provided by humans can also be ambiguous and lack precise details about specific locations, objects, or actions, exacerbating the hallucination issue. In this work, we introduce Seeing with Partial Certainty (SwPC) - a framework designed to measure and align uncertainty in VLM-based place recognition, enabling the model to recognize when it lacks confidence and seek assistance when necessary. This framework is built on the theory of conformal prediction to provide statistical guarantees on place recognition while minimizing requests for human help in complex indoor environment settings. Through experiments on the widely used richly-annotated scene dataset Matterport3D, we show that SwPC significantly increases the success rate and decreases the amount of human intervention required relative to the prior art. SwPC can be utilized with any VLMs directly without requiring model fine-tuning, offering a promising, lightweight approach to uncertainty modeling that complements and scales alongside the expanding capabilities of foundational models.

==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\hfill \break
The proposed shared-autonomy based navigation framework is designed to incorporate user preferences and user control into the navigation pipeline, thus improving the efficiency and safety of the navigation process. We discussed the structure of the UPF-based A* and adaptive shared-control based MPC local planner. The evaluation results indicate that this shared-autonomy based navigation framework can enhance efficiency and also generate a user-desired path.

Our insight is to use shared control to combine the advantages of autonomous navigation and the user's experience, yielding better performance than either alone. However, even though the application of shared control is promising in improving trust and safety, the current input methods and preference-taking from the user, which rely on clicking and tele-operation, can distract the user during navigation in a crowded indoor environment, increasing collision risks. Using EEG signals generated by the user, rather than tele-operation, offers a more seamless way for people to share their control intentions and path preferences with the robot \cite{EEG}. 

Additionally, our navigation framework builds on the assumption that users can gather sufficient information to decide their preferred route. To enable users to better understand the environment, it's crucial to build a topological semantic map that contains detailed environment information\cite{hughes2022hydra} and create a user-friendly GUI\cite{GUI} for tablet or VR device\cite{doi:10.1061/JMENEA.MEENG-5227}. These additions will be important considerations when we deploy this framework for real robot experimentation.
